The Dispersion Bias

Estimation error has plagued quantitative finance since Harry Markowitz launched modern portfolio theory in 1952. Using random matrix theory, we characterize a source of bias in the sample eigenvectors of financial covariance matrices. Unchecked, the bias distorts weights of minimum variance portfolios and leads to risk forecasts that are severely biased downward. To address these issues, we develop an eigenvector bias correction. Our approach is distinct from the regularization and eigenvalue shrinkage methods found in the literature. We provide theoretical guarantees on the improvement our correction provides as well as estimation methods for computing the optimal correction from data.

==> sections/cross_validation.tex <==
% -*- root: ../minvar.tex -*-

We introduce here a cross-validation method for computing an estimate of the
optimal shrinkage parameter $\rho^*$.  

\begin{itemize}
	\item principles: monte carlo train/test splits
	\begin{itemize}
		\item Independent train/test splits $X^{(k)}_{train}$, $X^{(k)}_{test}$

	\end{itemize}
	\item loss functions: negative log likelihood, var ratio, te
	\item results
\end{itemize}

==> sections/history.tex <==
% -*- root: ../minvar.tex -*-
In the community of finance practitioners, it is usual to shrink estimated market betas and there are two standard methods.  
The first method,  \cite{vasicek1973}, uses a Bayesian adjustment to shrink betas estimated with time-series regression toward their cross-sectional mean.
The second method,  \cite{blume1975},  uses the empirically observed average shrinkage of betas on individual stocks in the current period
relative to a previous period to adjust forecast betas for the next period.

==> sections/notation.tex <==
% -*- root: ../minvar.tex -*-


{\bf Notation.}
The notation \tq{$f \sim g$} denotes that $f$ and $g$ are equal
asymptotically.  Precisely, the limit $\lim_{x \upto \infty}
\frac{f\p{x}}{g\p{x}}$ exists and is equal to $1$.  We use
$\cas$ and $\stackrel{p}{\rightarrow}$ to denote convergence
almost surely and convergence in probability, respectively.


%The notation  \tq{$f \asymp g$} denotes that $f$ and $g$ are of
% the same magnitute asymptotically. Precisely, there exist
% constants $c,C>0$ and $x_0$ such that $c g\p{x} \le f\p{x} \le C
%g\p{x}$ for all $x \ge x_0$.  

\begin{comment}
The notation \tq{$f \sim g$} denotes that $f$ and $g$ are equal
asymptotically.  Precisely, the limit $\lim_{x \upto \infty}
\frac{f\p{x}}{g\p{x}}$ exists and is equal to $1$.  We use
$\cas$ and $\stackrel{p}{\rightarrow}$ to denote convergence
almost surely and convergence in probability, respectively.
\end{comment}



\begin{comment}
Our calibration is summarized in
Table~\ref{table:cal}.


 \begin{table}[h]
 	\begin{center}
 		\begin{tabular}{l l l c}
 		 %\hline
 		% \multicolumn{4}{|c|}{Description of Factors} \\
 		\toprule
 		{\bf Parameter} & {\bf Value} & {\bf Comment}\\
 		\midrule
		$\nv$ &  500--3000&  number of securities \\ \\
		$\no$  &   250 &  number of observations  \\ \\
		$B$       & first column drawn from ${\cal N}(1, \tau^2)$&  matrix of factor exposures \\ 
				     &columns 2, 3 and 4 drawn from ${\cal N}(0,1)$ \\ 
		     &columns normalized to $L_2$  length 1  \\ \\
		 $\beta$ &   &  first column of $B$ \\ \\
 		$\gamma_{\beta, z}$ &  0.5--1.0 & controls dominant\\
 		&& factor concentration \ \\
 		$\vf$ & $(0.16)^2\nv (1 + \tau^2)$&  calibrated to
market \\
 		           &&volatility of 16\%\\  \\
 		$\vs_n$ &   specific variances  & annualized specific\\
 		    && volatilities drawn\\
 		    && from $[10\%, 64\%]$\\
 		\bottomrule
 		\end{tabular}
 		\caption{Calibration of the one-factor model  used to simulate security returns.
 		\label{table:cal}}
 	\end{center}
 \end{table} 

 \begin{table}[h]
 	\begin{center}
 		\begin{tabular}{l c l c}
 		 %\hline
 		% \multicolumn{4}{|c|}{Description of Factors} \\
 		\toprule
 		{\bf Parameter} & {\bf Value} & {\bf Comment}\\
 		\midrule
 		$\beta$ & normalized so $||\beta||_2 = 1$ & factor exposure\\ \\
 		$\gamma_{\beta, z}$ &  0.5--1.0 & controls dominant\\
 		&& factor dispersion\\ \\
 		$\vf$ & scaled factor variance&  calibrated to
market \\
 		           &&volatility of 16\%\\  \\
 		$\vs_n$ &   specific variances  & annualized specific\\
 		    && volatilities drawn\\
 		    && from $[10\%, 64\%]$\\
 		\bottomrule
 		\end{tabular}
 		\caption{Calibration of the one-factor model  used to simulate security returns.
 		\label{table:cal}}
 	\end{center}
 \end{table} 
 \end{comment}


==> sections/organization.tex <==
% -*- root: ../minvar.tex -*-



==> tables/multifactor_lowrisk/table_N.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 1.10\% & 0.80\% & 0.76\% & 0.69\% & 0.74\% & 0.70\% \\
Oracle      & 0.80\% & 0.48\% & 0.37\% & 0.35\% & 0.33\% & 0.28\% \\
Data-Driven & 0.82\% & 0.49\% & 0.37\% & 0.35\% & 0.32\% & 0.28\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 2.93\% & 1.99\% & 1.68\% & 1.45\% & 1.39\% & 1.27\% \\
Oracle      & 2.83\% & 1.89\% & 1.54\% & 1.32\% & 1.22\% & 1.10\% \\
Data-Driven & 2.83\% & 1.89\% & 1.54\% & 1.32\% & 1.22\% & 1.10\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.854 & 0.811 & 0.761 & 0.737 & 0.680 & 0.663 \\
Oracle      & 0.995 & 0.979 & 0.974 & 0.981 & 0.962 & 0.965 \\
Data-Driven & 0.991 & 0.974 & 0.970 & 0.969 & 0.960 & 0.960 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 1.002 & 0.986 & 0.982 & 1.002 & 0.978 & 1.002 \\
Oracle      & 1.002 & 0.986 & 0.982 & 1.002 & 0.978 & 1.002 \\
Data-Driven & 1.002 & 0.986 & 0.982 & 1.002 & 0.978 & 1.002 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/multifactor_lowrisk/table_gam.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.25\% & 0.35\% & 0.40\% & 0.58\% & 1.10\% & 1.97\% & 9.09\% \\
Oracle      & 0.23\% & 0.31\% & 0.35\% & 0.49\% & 0.80\% & 1.42\% & 0.54\% \\
Data-Driven & 0.24\% & 0.33\% & 0.37\% & 0.50\% & 0.82\% & 1.43\% & 3.10\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &   1.00 \\
\midrule
PCA         & 1.34\% & 1.53\% & 1.68\% & 1.89\% & 2.93\% & 4.18\% & 20.17\% \\
Oracle      & 1.33\% & 1.52\% & 1.66\% & 1.87\% & 2.83\% & 3.95\% & 18.02\% \\
Data-Driven & 1.33\% & 1.52\% & 1.67\% & 1.87\% & 2.83\% & 3.95\% & 18.27\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.985 & 0.959 & 0.952 & 0.898 & 0.854 & 0.725 & 0.255 \\
Oracle      & 1.015 & 0.994 & 0.993 & 0.982 & 0.995 & 0.970 & 1.020 \\
Data-Driven & 1.011 & 0.992 & 0.987 & 0.968 & 0.991 & 0.957 & 0.928 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 1.029 & 1.015 & 0.995 & 1.003 & 1.002 & 1.003 & 1.021 \\
Oracle      & 1.029 & 1.015 & 0.995 & 1.003 & 1.002 & 1.003 & 1.021 \\
Data-Driven & 1.030 & 1.015 & 0.995 & 1.003 & 1.002 & 1.003 & 1.021 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/onefactor_fattails_lowrisk/table_N.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.98\% & 0.90\% & 0.75\% & 0.79\% & 0.70\% & 0.74\% \\
Oracle      & 0.83\% & 0.62\% & 0.48\% & 0.45\% & 0.38\% & 0.36\% \\
Data-Driven & 0.85\% & 0.63\% & 0.49\% & 0.46\% & 0.39\% & 0.37\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 2.83\% & 2.08\% & 1.68\% & 1.57\% & 1.37\% & 1.32\% \\
Oracle      & 2.78\% & 1.98\% & 1.58\% & 1.43\% & 1.24\% & 1.16\% \\
Data-Driven & 2.79\% & 1.98\% & 1.59\% & 1.43\% & 1.24\% & 1.16\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.743 & 0.689 & 0.679 & 0.626 & 0.637 & 0.587 \\
Oracle      & 0.828 & 0.827 & 0.819 & 0.820 & 0.826 & 0.820 \\
Data-Driven & 0.830 & 0.821 & 0.813 & 0.819 & 0.822 & 0.820 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 1.014 & 0.971 & 0.984 & 0.989 & 1.002 &  0.96 \\
Oracle      & 1.014 & 0.971 & 0.984 & 0.989 & 1.002 &  0.96 \\
Data-Driven & 1.014 & 0.971 & 0.984 & 0.989 & 1.002 &  0.96 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/onefactor_fattails_lowrisk/table_gam.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.39\% & 0.41\% & 0.51\% & 0.61\% & 0.98\% & 1.79\% & 8.79\% \\
Oracle      & 0.37\% & 0.38\% & 0.48\% & 0.54\% & 0.83\% & 1.48\% & 0.37\% \\
Data-Driven & 0.37\% & 0.39\% & 0.48\% & 0.55\% & 0.85\% & 1.51\% & 1.41\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &   1.00 \\
\midrule
PCA         & 1.41\% & 1.47\% & 1.79\% & 2.01\% & 2.83\% & 4.18\% & 19.57\% \\
Oracle      & 1.41\% & 1.46\% & 1.78\% & 1.99\% & 2.78\% & 4.05\% & 17.49\% \\
Data-Driven & 1.41\% & 1.46\% & 1.78\% & 2.00\% & 2.79\% & 4.07\% & 17.54\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.809 & 0.807 & 0.789 & 0.780 & 0.743 & 0.678 & 0.263 \\
Oracle      & 0.833 & 0.839 & 0.827 & 0.824 & 0.828 & 0.829 & 1.011 \\
Data-Driven & 0.829 & 0.832 & 0.822 & 0.821 & 0.830 & 0.820 & 0.997 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 1.018 & 0.979 & 1.007 & 1.024 & 1.014 & 1.013 & 1.012 \\
Oracle      & 1.018 & 0.979 & 1.007 & 1.024 & 1.014 & 1.014 & 1.012 \\
Data-Driven & 1.019 & 0.979 & 1.007 & 1.024 & 1.014 & 1.014 & 1.012 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/onefactor_highrisk/table_N.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 2.20\% & 2.08\% & 2.18\% & 1.99\% & 1.97\% & 1.97\% \\
Oracle      & 1.50\% & 1.09\% & 0.96\% & 0.80\% & 0.70\% & 0.66\% \\
Data-Driven & 1.52\% & 1.11\% & 0.97\% & 0.81\% & 0.72\% & 0.67\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 4.97\% & 3.85\% & 3.48\% & 3.05\% & 2.84\% & 2.73\% \\
Oracle      & 4.71\% & 3.42\% & 2.87\% & 2.44\% & 2.17\% & 2.00\% \\
Data-Driven & 4.71\% & 3.43\% & 2.88\% & 2.45\% & 2.17\% & 2.01\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.723 & 0.633 & 0.535 & 0.512 & 0.460 & 0.425 \\
Oracle      & 0.981 & 0.981 & 0.983 & 0.983 & 0.982 & 0.983 \\
Data-Driven & 0.974 & 0.980 & 0.980 & 0.982 & 0.974 & 0.978 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 1.001 & 0.996 & 0.984 & 0.999 & 0.983 &  1.01 \\
Oracle      & 1.001 & 0.996 & 0.985 & 0.999 & 0.983 &  1.01 \\
Data-Driven & 1.001 & 0.996 & 0.985 & 0.999 & 0.983 &  1.01 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/onefactor_highrisk/table_gam.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.43\% & 0.59\% & 0.81\% & 1.17\% & 2.20\% & 3.72\% & 8.23\% \\
Oracle      & 0.31\% & 0.40\% & 0.54\% & 0.76\% & 1.50\% & 2.74\% & 0.21\% \\
Data-Driven & 0.33\% & 0.41\% & 0.56\% & 0.79\% & 1.52\% & 2.75\% & 1.15\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &   1.00 \\
\midrule
PCA         & 2.38\% & 2.64\% & 2.95\% & 3.54\% & 4.97\% & 7.05\% & 19.43\% \\
Oracle      & 2.36\% & 2.60\% & 2.89\% & 3.43\% & 4.71\% & 6.59\% & 17.60\% \\
Data-Driven & 2.36\% & 2.60\% & 2.90\% & 3.44\% & 4.71\% & 6.59\% & 17.64\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.946 & 0.917 & 0.889 & 0.840 & 0.723 & 0.595 & 0.269 \\
Oracle      & 0.985 & 0.984 & 0.984 & 0.984 & 0.981 & 0.982 & 0.997 \\
Data-Driven & 0.983 & 0.977 & 0.982 & 0.981 & 0.974 & 0.969 & 0.981 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 1.035 & 1.006 & 1.017 & 1.012 & 1.001 & 0.982 & 0.998 \\
Oracle      & 1.035 & 1.007 & 1.017 & 1.012 & 1.001 & 0.982 & 0.998 \\
Data-Driven & 1.035 & 1.007 & 1.017 & 1.012 & 1.001 & 0.982 & 0.998 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/onefactor_lowrisk/table_N.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.89\% & 0.85\% & 0.69\% & 0.77\% & 0.71\% & 0.74\% \\
Oracle      & 0.61\% & 0.43\% & 0.32\% & 0.30\% & 0.26\% & 0.25\% \\
Data-Driven & 0.62\% & 0.44\% & 0.33\% & 0.31\% & 0.27\% & 0.26\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 2.80\% & 2.06\% & 1.66\% & 1.56\% & 1.38\% & 1.32\% \\
Oracle      & 2.73\% & 1.93\% & 1.54\% & 1.39\% & 1.21\% & 1.13\% \\
Data-Driven & 2.73\% & 1.93\% & 1.54\% & 1.39\% & 1.21\% & 1.13\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.854 & 0.789 & 0.795 & 0.715 & 0.698 & 0.653 \\
Oracle      & 0.983 & 0.980 & 0.983 & 0.982 & 0.985 & 0.982 \\
Data-Driven & 0.985 & 0.977 & 0.981 & 0.981 & 0.981 & 0.980 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrr}
\toprule
N &  500  &  1000 &  1500 &  2000 &  2500 &  3000 \\
\midrule
PCA         & 0.996 & 0.988 & 1.019 &  0.99 & 1.019 & 0.986 \\
Oracle      & 0.996 & 0.988 & 1.019 &  0.99 & 1.019 & 0.986 \\
Data-Driven & 0.996 & 0.988 & 1.019 &  0.99 & 1.019 & 0.986 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}


==> tables/onefactor_lowrisk/table_gam.tex <==

\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.18\% & 0.22\% & 0.32\% & 0.42\% & 0.89\% & 1.79\% & 8.34\% \\
Oracle      & 0.15\% & 0.17\% & 0.23\% & 0.30\% & 0.61\% & 1.19\% & 0.21\% \\
Data-Driven & 0.17\% & 0.18\% & 0.25\% & 0.31\% & 0.62\% & 1.21\% & 1.15\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Tracking Error: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &   1.00 \\
\midrule
PCA         & 1.37\% & 1.42\% & 1.75\% & 1.96\% & 2.80\% & 4.18\% & 19.37\% \\
Oracle      & 1.37\% & 1.42\% & 1.73\% & 1.94\% & 2.73\% & 3.96\% & 17.49\% \\
Data-Driven & 1.37\% & 1.42\% & 1.73\% & 1.94\% & 2.73\% & 3.96\% & 17.52\% \\
\bottomrule
\end{tabular}

    \caption{Annualized Volatility: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.970 & 0.954 & 0.941 & 0.925 & 0.854 & 0.746 & 0.272 \\
Oracle      & 0.992 & 0.999 & 0.993 & 0.987 & 0.983 & 0.973 & 1.027 \\
Data-Driven & 0.994 & 0.993 & 0.985 & 0.984 & 0.985 & 0.972 & 1.014 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Minimum Variance}
\end{subtable}


\begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lrrrrrrr}
\toprule
$\gamma_{\beta, z}$ &  0.50 &  0.60 &  0.70 &  0.80 &  0.90 &  0.95 &  1.00 \\
\midrule
PCA         & 0.997 & 1.010 & 1.022 & 0.997 & 0.996 &   1.0 & 1.027 \\
Oracle      & 0.997 & 1.011 & 1.022 & 0.997 & 0.996 &   1.0 & 1.027 \\
Data-Driven & 0.997 & 1.011 & 1.022 & 0.997 & 0.996 &   1.0 & 1.027 \\
\bottomrule
\end{tabular}

    \caption{Forecast Ratio: Equal Weighted}
\end{subtable}

